Optimizing Optimizations, Declaratively: Optimizing the Higher-Order Functions in Mathematical Optimization with egglog

We present two applications of egglog to mathematical optimization in JijModeling 2, a mathematical modeller whose internal representation is based on simply typed $\lambda$-calculus. First, we use egglog to improve $\LaTeX$ output for mathematical models expressed with higher-order functions. Python comprehensions are desugared into stream operations such as $\textsf{map}$, $\textsf{flat_map}$, and $\textsf{filter}$; emitting these terms directly produces unnatural mathematical notation. We reconstruct comprehension syntax by \emph{ensugaring} higher-order terms and use equality saturation with a custom cost model to minimize temporary variable rebindings. Second, we use egglog as a declarative engine for \emph{constraint detection}, extending the previous egg-based approach presented at EGRAPHS '25. Egglog's datalog-style rules let us express multi-step detection logic directly, without external Rust orchestration code. We encode parametrized constraints using \emph{Henkin-like constants} and propagate side conditions on subterms and indices through egglog facts. Finally, we show that the same ensugaring procedure also reduces large domain-set conditions before saturation, turning a problematic detection case from minutes or nontermination into a few seconds. Through these topics, we want to provide an example of an industrial application of egglog, demonstrate the trick to propagate the constraints using the ideas from mathematical logic, and show the importance of optimizing \emph{premises} of egglog rules to get practical performance in egglog programs.

==> grammar.ott.tex <==
% generated by Ott 0.34 from: ott/grammar.ott
\newcommand{\ottdrule}[4][]{{\displaystyle\frac{\begin{array}{l}#2\end{array}}{#3}\quad\ottdrulename{#4}}}
\newcommand{\ottusedrule}[1]{\[#1\]}
\newcommand{\ottpremise}[1]{ #1 \\}
\newenvironment{ottdefnblock}[3][]{ \framebox{\mbox{#2}} \quad #3 \\[0pt]}{}
\newenvironment{ottfundefnblock}[3][]{ \framebox{\mbox{#2}} \quad #3 \\[0pt]\begin{displaymath}\begin{array}{l}}{\end{array}\end{displaymath}}
\newcommand{\ottfunclause}[2]{ #1 \equiv #2 \\}
\newcommand{\ottnt}[1]{\mathit{#1}}
\newcommand{\ottmv}[1]{\mathit{#1}}
\newcommand{\ottkw}[1]{\mathbf{#1}}
\newcommand{\ottsym}[1]{#1}
\newcommand{\ottcom}[1]{\text{#1}}
\newcommand{\ottdrulename}[1]{\textsc{#1}}
\newcommand{\ottcomplu}[5]{\overline{#1}^{\,#2\in #3 #4 #5}}
\newcommand{\ottcompu}[3]{\overline{#1}^{\,#2<#3}}
\newcommand{\ottcomp}[2]{\overline{#1}^{\,#2}}
\newcommand{\ottgrammartabular}[1]{\begin{supertabular}{llcllllll}#1\end{supertabular}}
\newcommand{\ottmetavartabular}[1]{\begin{supertabular}{ll}#1\end{supertabular}}
\newcommand{\ottrulehead}[3]{$#1$ & & $#2$ & & & \multicolumn{2}{l}{#3}}
\newcommand{\ottprodline}[6]{& & $#1$ & $#2$ & $#3 #4$ & $#5$ & $#6$}
\newcommand{\ottfirstprodline}[6]{\ottprodline{#1}{#2}{#3}{#4}{#5}{#6}}
\newcommand{\ottlongprodline}[2]{& & $#1$ & \multicolumn{4}{l}{$#2$}}
\newcommand{\ottfirstlongprodline}[2]{\ottlongprodline{#1}{#2}}
\newcommand{\ottbindspecprodline}[6]{\ottprodline{#1}{#2}{#3}{#4}{#5}{#6}}
\newcommand{\ottprodnewline}{\\}
\newcommand{\ottinterrule}{\\[5.0mm]}
\newcommand{\ottafterlastrule}{\\}
\newcommand{\ottmetavars}{
\ottmetavartabular{
 $ \mathit{freevar} ,\, \mathit{a} ,\, \mathit{b} ,\, \plural{a} ,\, \plural{b} $ & \ottcom{free variable} \\
 $ \ottmv{index} ,\, \ottmv{n} ,\, \ottmv{k} ,\, k + 1 ,\, \ottmv{i} $ &  \\
 $ \mathit{boundvar} ,\, x ,\, \plural{x} $ & \ottcom{bound variable} \\
 $ \mathit{string} ,\, \mathit{str} $ & \ottcom{string constant} \\
 $ \mathit{natural} ,\, \mathit{N} $ & \ottcom{natural number constant} \\
 $ \mathit{label} ,\, \ell $ & \ottcom{label name} \\
 $ \mathit{real} ,\, c $ & \ottcom{real constant} \\
}}

\newcommand{\ottprimop}{
\ottrulehead{\ottnt{primop}  ,\ \ottnt{f}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \textsf{add} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \textsf{div} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ldots }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \textsf{map} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \textsf{flat\_map} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \textsf{filter} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ldots }{}{}{}{}}

\newcommand{\ottexpr}{
\ottrulehead{\ottnt{expr}  ,\ \ottnt{e}}{::=}{\ottcom{term}}\ottprodnewline
\ottfirstprodline{|}{\mathit{a}}{}{}{}{\ottcom{free var}}\ottprodnewline
\ottprodline{|}{x_{\ottmv{i}}}{}{}{}{\ottcom{bound var}}\ottprodnewline
\ottprodline{|}{ \ottnt{e} _{e_1, \ldots, e_n} }{}{}{}{\ottcom{subscript}}\ottprodnewline
\ottprodline{|}{ \lambda  \ottnt{p} \ldotp  \ottnt{e} }{}{}{}{\ottcom{lambda}}\ottprodnewline
\ottprodline{|}{\ottnt{f}  \ottsym{(}  \ottnt{e_{{\mathrm{1}}}}  \ottsym{,} \, .. \, \ottsym{,}  \ottnt{e_{\ottmv{n}}}  \ottsym{)}}{}{}{}{\ottcom{primops}}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \ottnt{e_{{\mathrm{1}}}}  \ottsym{,} \, .. \, \ottsym{,}  \ottnt{e_{\ottmv{n}}}  \ottsym{)}}{}{}{}{\ottcom{tuple}}\ottprodnewline
\ottprodline{|}{\ottsym{[}  \ottnt{e_{{\mathrm{1}}}}  \ottsym{,} \, .. \, \ottsym{,}  \ottnt{e_{\ottmv{n}}}  \ottsym{]}}{}{}{}{\ottcom{list}}\ottprodnewline
\ottprodline{|}{\ottnt{e} \, \ottnt{e'}}{}{}{}{\ottcom{app}}}

\newcommand{\ottcompr}{
\ottrulehead{\ottnt{compr}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ [\  \ottnt{e}  \mid   \plural{C}  \ ] }{}{}{}{}}

\newcommand{\ottcomprClauses}{
\ottrulehead{\mathit{compclss}  ,\ \plural{C}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathit{forcls}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \plural{C}  ;\   \ottnt{C} }{}{}{}{}}

\newcommand{\ottforClause}{
\ottrulehead{\mathit{forcls}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \textbf{for }  \ottnt{p}  \ \textbf{in }  \ottnt{e} }{}{}{}{}}

\newcommand{\ottcomprClause}{
\ottrulehead{\mathit{compcls}  ,\ \ottnt{C}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathit{forcls}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \textbf{if }  \ottnt{e} }{}{}{}{}}

\newcommand{\ottextendedXXcomprehension}{
\ottrulehead{\ottnt{extended\_comprehension}}{::=}{\ottcom{comprehension}}\ottprodnewline
\ottfirstprodline{|}{ [ \  \ottnt{e}  \mid  \ottnt{for\_if\_let\_clauses}  \ ] }{}{}{}{\ottcom{list comprehension}}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \ottnt{e} \, \ottnt{for\_if\_let\_clauses}  \ottsym{)}}{}{}{}{\ottcom{generator expression}}}

\newcommand{\ottforXXifXXletXXclauses}{
\ottrulehead{\ottnt{for\_if\_let\_clauses}  ,\ \plural{\kappa}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathit{forcls}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{for\_if\_let\_clauses} ;\  \ottnt{for\_if\_let\_clause} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \plural{\kappa} ;\  \plural{\kappa}' }{}{}{}{}}

\newcommand{\ottforXXifXXletXXclause}{
\ottrulehead{\ottnt{for\_if\_let\_clause}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathit{forcls}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \textbf{if }  \ottnt{e} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \textbf{let }  \ottnt{p}  =  \ottnt{e} }{}{}{}{}}

\newcommand{\ottpattern}{
\ottrulehead{\ottnt{pattern}  ,\ \ottnt{p}}{::=}{\ottcom{pattern}}\ottprodnewline
\ottfirstprodline{|}{x_{\ottmv{i}}}{}{}{}{\ottcom{bound var}}\ottprodnewline
\ottprodline{|}{\mathit{a}}{}{}{}{\ottcom{free var}}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \ottnt{p_{{\mathrm{1}}}}  \ottsym{,} \, .. \, \ottsym{,}  \ottnt{p_{\ottmv{n}}}  \ottsym{)}}{}{}{}{\ottcom{tuple}}}

\newcommand{\ottscalar}{
\ottrulehead{\ottnt{scalar}  ,\ \alpha}{::=}{\ottcom{domain of scalar}}\ottprodnewline
\ottfirstprodline{|}{ \mathbb{R} }{}{}{}{\ottcom{real}}\ottprodnewline
\ottprodline{|}{ \mathbb{Z} }{}{}{}{\ottcom{integer}}\ottprodnewline
\ottprodline{|}{ \mathbb{N} }{}{}{}{\ottcom{natural number}}\ottprodnewline
\ottprodline{|}{ \set{0, 1} }{}{}{}{\ottcom{binary (i.e. 0 or 1)}}}

\newcommand{\ottintegral}{
\ottrulehead{\ottnt{integral}  ,\ \iota}{::=}{\ottcom{integral scalars}}\ottprodnewline
\ottfirstprodline{|}{ \mathbb{Z} }{}{}{}{\ottcom{integer}}\ottprodnewline
\ottprodline{|}{ \mathbb{N} }{}{}{}{\ottcom{natural number}}\ottprodnewline
\ottprodline{|}{ \set{0, 1} }{}{}{}{\ottcom{binary (i.e. 0 or 1)}}}

\newcommand{\ottstage}{
\ottrulehead{\ottnt{stage}  ,\ \mu}{::=}{\ottcom{stage of scalar}}\ottprodnewline
\ottfirstprodline{|}{ \dyn }{}{}{}{\ottcom{dynamic (may contain decision variables)}}\ottprodnewline
\ottprodline{|}{ \stat }{}{}{}{\ottcom{static (doesn't contain decision variables)}}}

\newcommand{\ottdimspec}{
\ottrulehead{\ottnt{dimspec}  ,\ \delta}{::=}{\ottcom{dimension specification}}\ottprodnewline
\ottfirstprodline{|}{ \RangeNat{ \ottnt{e} } }{}{}{}{\ottcom{fixed size}}\ottprodnewline
\ottprodline{|}{ ? }{}{}{}{\ottcom{unknown size}}}

\newcommand{\ottdims}{
\ottrulehead{\ottnt{dims}  ,\ \plural{\delta}}{::=}{\ottcom{dimensions}}\ottprodnewline
\ottfirstprodline{|}{ \delta }{}{}{}{\ottcom{singleton dimension}}\ottprodnewline
\ottprodline{|}{ \delta  ,  \ottnt{dims} }{}{}{}{\ottcom{extend dimensions}}\ottprodnewline
\ottprodline{|}{ \delta  , \ldots ,  \delta' }{}{}{}{\ottcom{n-many dimensions}}}

\newcommand{\ottcomparison}{
\ottrulehead{\ottnt{comparison}  ,\ \lesseqgtr}{::=}{\ottcom{comparison operators}}\ottprodnewline
\ottfirstprodline{|}{ < }{}{}{}{\ottcom{less than}}\ottprodnewline
\ottprodline{|}{ \leq }{}{}{}{\ottcom{less than or equal to}}\ottprodnewline
\ottprodline{|}{ = }{}{}{}{\ottcom{equal to}}\ottprodnewline
\ottprodline{|}{ \neq }{}{}{}{\ottcom{not equal to}}\ottprodnewline
\ottprodline{|}{ \geq }{}{}{}{\ottcom{greater than or equal to}}\ottprodnewline
\ottprodline{|}{ > }{}{}{}{\ottcom{greater than}}}

\newcommand{\otttype}{
\ottrulehead{\ottnt{type}  ,\ \ottnt{T}  ,\ \ottnt{U}}{::=}{\ottcom{type}}\ottprodnewline
\ottfirstprodline{|}{\ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}}{}{}{}{\ottcom{function type}}\ottprodnewline
\ottprodline{|}{ (T_1 \times \cdots \times T_n) }{}{}{}{\ottcom{tuple type}}\ottprodnewline
\ottprodline{|}{ \Comp{ \ottnt{T_{{\mathrm{1}}}} }{ \lesseqgtr }{ \ottnt{T_{{\mathrm{2}}}} } }{}{}{}{\ottcom{comparison type between $\ottnt{T_{{\mathrm{1}}}}$ and $\ottnt{T_{{\mathrm{2}}}}$}}\ottprodnewline
\ottprodline{|}{ \Scalar{ \mu }{ \alpha } }{}{}{}{\ottcom{scalar type with stage and domain}}\ottprodnewline
\ottprodline{|}{ \RangeNat{ \ottnt{e} } }{}{}{}{\ottcom{natural numbers less than $\ottnt{e}$}}\ottprodnewline
\ottprodline{|}{ \mathbb{B} }{}{}{}{\ottcom{boolean}}\ottprodnewline
\ottprodline{|}{\ottkw{String}}{}{}{}{\ottcom{string}}\ottprodnewline
\ottprodline{|}{ \ottnt{T} ^{ \plural{\delta} } }{}{}{}{\ottcom{Array type}}\ottprodnewline
\ottprodline{|}{ \SetOf{ \ottnt{T} } }{}{}{}{\ottcom{set (stream) of $\ottnt{T}$s}}\ottprodnewline
\ottprodline{|}{ \PromotedSet{ \ottnt{e} } }{}{}{}{\ottcom{element of set-expression $\ottnt{e}$}}\ottprodnewline
\ottprodline{|}{ \CatLab{ \ell } }{}{}{}{\ottcom{opaque category label \ell}}\ottprodnewline
\ottprodline{|}{ \TotalDict{ \ottnt{K} }{ \ottnt{T} } }{}{}{}{\ottcom{total dictionary from $\ottnt{K}$ to $\ottnt{T}$}}\ottprodnewline
\ottprodline{|}{ \PartialDict{ \ottnt{K} }{ \ottnt{T} } }{}{}{}{\ottcom{partial dictionary from $\ottnt{K}$ to $\ottnt{T}$}}}

\newcommand{\ottonlystat}{
\ottrulehead{\stat}{::=}{\ottcom{only static stage}}\ottprodnewline
\ottfirstprodline{|}{ \stat }{}{}{}{\ottcom{static (doesn't contain decision variables)}}}

\newcommand{\ottkeytype}{
\ottrulehead{\ottnt{keytype}  ,\ \ottnt{K}}{::=}{\ottcom{key type for dictionaries}}\ottprodnewline
\ottfirstprodline{|}{ \Scalar{ \stat }{ \alpha } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ (T_1 \times \cdots \times T_n) }{}{}{}{\ottcom{tuple key type}}}

\newcommand{\ottcontext}{
\ottrulehead{\ottnt{context}  ,\ \Gamma}{::=}{\ottcom{typing context}}\ottprodnewline
\ottfirstprodline{|}{ \emptyset }{}{}{}{\ottcom{empty context}}\ottprodnewline
\ottprodline{|}{ \mathit{ \mathit{a} } :  \ottnt{T} ,  \Gamma }{}{}{}{\ottcom{extend context}}\ottprodnewline
\ottprodline{|}{ D \left\{  \ottnt{p}  :  \ottnt{T}  \right\} ,  \Gamma }{}{}{}{\ottcom{extend context with pattern}}}

\newcommand{\otttypestack}{
\ottrulehead{\ottnt{typestack}  ,\ \Psi}{::=}{\ottcom{type stack}}\ottprodnewline
\ottfirstprodline{|}{ \emptyset }{}{}{}{\ottcom{empty type stack}}\ottprodnewline
\ottprodline{|}{ \ottnt{T} }{}{}{}{\ottcom{singleton type stack}}\ottprodnewline
\ottprodline{|}{ \Psi  ,  \ottnt{T} }{}{}{}{\ottcom{extend type stack}}}

\newcommand{\otttyexpr}{
\ottrulehead{\ottnt{tyexpr}  ,\ T}{::=}{\ottcom{type expressions}}\ottprodnewline
\ottfirstprodline{|}{\ottnt{T}}{}{}{}{\ottcom{type}}\ottprodnewline
\ottprodline{|}{ \ottnt{T}  \land  T }{}{}{}{\ottcom{type intersection}}\ottprodnewline
\ottprodline{|}{ \ottnt{T_{{\mathrm{1}}}}  \lor \ldots \lor  \ottnt{T_{{\mathrm{2}}}} }{}{}{}{\ottcom{n-ary type sup}}\ottprodnewline
\ottprodline{|}{ \ottnt{T}  \lor  T }{}{}{}{\ottcom{type union}}}

\newcommand{\ottscalarexpr}{
\ottrulehead{\ottnt{scalarexpr}  ,\ \alpha}{::=}{\ottcom{stage expressions}}\ottprodnewline
\ottfirstprodline{|}{\alpha}{}{}{}{\ottcom{scalar}}\ottprodnewline
\ottprodline{|}{ \alpha  \lor  \ottnt{scalarexpr} }{}{}{}{\ottcom{stage union}}\ottprodnewline
\ottprodline{|}{ \alpha  \land  \ottnt{scalarexpr} }{}{}{}{\ottcom{stage intersection}}}

\newcommand{\ottstageexpr}{
\ottrulehead{\ottnt{stageexpr}  ,\ \mu}{::=}{\ottcom{stage expressions}}\ottprodnewline
\ottfirstprodline{|}{\mu}{}{}{}{\ottcom{stage}}\ottprodnewline
\ottprodline{|}{ \mu  \lor  \ottnt{stageexpr} }{}{}{}{\ottcom{stage union}}\ottprodnewline
\ottprodline{|}{ \mu  \land  \ottnt{stageexpr} }{}{}{}{\ottcom{stage intersection}}}

\newcommand{\ottdimsubexpr}{
\ottrulehead{\ottnt{dimsubexpr}  ,\ \mu}{::=}{\ottcom{stage expressions}}\ottprodnewline
\ottfirstprodline{|}{\delta}{}{}{}{\ottcom{stage}}\ottprodnewline
\ottprodline{|}{ \delta  \lor  \ottnt{dimsubexpr} }{}{}{}{\ottcom{dim union}}\ottprodnewline
\ottprodline{|}{ \delta  \land  \ottnt{dimsubexpr} }{}{}{}{\ottcom{dim intersection}}}

\newcommand{\ottdestructor}{
\ottrulehead{\ottnt{destructor}  ,\ \ottnt{D}}{::=}{\ottcom{destructors for pattern matching}}\ottprodnewline
\ottfirstprodline{|}{ \left(x_{ \ottmv{i} } :  \ottnt{T}  \right) }{}{}{}{\ottcom{bind a value of type $\ottnt{T}$ as $\ottmv{i}$-th variable}}\ottprodnewline
\ottprodline{|}{ \mathbf{tuple}_{D_1, \ldots, D_n} }{}{}{}{\ottcom{splitting as a tuple}}\ottprodnewline
\ottprodline{|}{ \mathbf{Array}_{D_1, \ldots, D_n} }{}{}{}{\ottcom{splitting as an array along the first axis}}}

\newcommand{\ottmonomial}{
\ottrulehead{\ottnt{monomial}  ,\ \ottnt{M}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{c \, x_{{\mathrm{1}}} \, ... \, x_{\ottmv{k}}}{}{}{}{}}

\newcommand{\ottfunction}{
\ottrulehead{\ottnt{function}  ,\ \varphi}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottnt{M_{{\mathrm{1}}}}  \ottsym{+} \, ... \, \ottsym{+}  \ottnt{M_{\ottmv{n}}}}{}{}{}{}}

\newcommand{\ottsense}{
\ottrulehead{\ottnt{sense}  ,\ S}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ {\min} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\max} }{}{}{}{}}

\newcommand{\ottdvkind}{
\ottrulehead{\ottnt{dvkind}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \mathbb{R} \mid \mathbb{Z} \mid \set{0, 1} \mid \dots }{}{}{}{}}

\newcommand{\ottdecvars}{
\ottrulehead{\ottnt{decvars}  ,\ \plural{\delta}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \emptyset }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \plural{\delta}  ,  \ottnt{decvar} }{}{}{}{}}

\newcommand{\ottdecvar}{
\ottrulehead{\ottnt{decvar}  ,\ \delta}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ x_{\ottmv{i}}  :  \ottnt{dvkind}  \cap [  c  ,  c'  ] }{}{}{}{}}

\newcommand{\ottconstraint}{
\ottrulehead{\ottnt{constraint}  ,\ \kappa}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \varphi  = 0 }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \varphi  \leq 0 }{}{}{}{}}

\newcommand{\ottconstraints}{
\ottrulehead{\plural{\kappa}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \emptyset }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \plural{a}  ,  \kappa }{}{}{}{}}

\newcommand{\ottinstance}{
\ottrulehead{\ottnt{instance}  ,\ \ottnt{I}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \mathbf{Instance}( S ,  \plural{\delta} ,  \plural{\kappa} ,  \varphi ) }{}{}{}{}}

\newcommand{\ottgrammar}{\ottgrammartabular{
\ottprimop\ottinterrule
\ottexpr\ottinterrule
\ottcompr\ottinterrule
\ottcomprClauses\ottinterrule
\ottforClause\ottinterrule
\ottcomprClause\ottinterrule
\ottextendedXXcomprehension\ottinterrule
\ottforXXifXXletXXclauses\ottinterrule
\ottforXXifXXletXXclause\ottinterrule
\ottpattern\ottinterrule
\ottscalar\ottinterrule
\ottintegral\ottinterrule
\ottstage\ottinterrule
\ottdimspec\ottinterrule
\ottdims\ottinterrule
\ottcomparison\ottinterrule
\otttype\ottinterrule
\ottonlystat\ottinterrule
\ottkeytype\ottinterrule
\ottcontext\ottinterrule
\otttypestack\ottinterrule
\otttyexpr\ottinterrule
\ottscalarexpr\ottinterrule
\ottstageexpr\ottinterrule
\ottdimsubexpr\ottinterrule
\ottdestructor\ottinterrule
\ottmonomial\ottinterrule
\ottfunction\ottinterrule
\ottsense\ottinterrule
\ottdvkind\ottinterrule
\ottdecvars\ottinterrule
\ottdecvar\ottinterrule
\ottconstraint\ottinterrule
\ottconstraints\ottinterrule
\ottinstance\ottafterlastrule
}}

% defnss
% defns Equality
%% defn dimeqv

\newcommand{\ottdefnEqXXdimeqv}[1]{\begin{ottdefnblock}[#1]{$\Gamma  \vdash  \delta  \sim  \delta'$}{\ottcom{$\delta$ is equal to $\delta'$}}
\end{ottdefnblock}}

%% defn scequiv
\newcommand{\ottdruleEqXXSclXXSupBin}[1]{\ottdrule[#1]{%
}{
  \set{0, 1}   \lor  \alpha   \sim  \alpha}{%
{\ottdrulename{Eq\_Scl\_SupBin}}{}%
}}


\newcommand{\ottdruleEqXXSclXXSupNat}[1]{\ottdrule[#1]{%
}{
  \mathbb{N}   \lor  \alpha   \sim   \mathbb{N} }{%
{\ottdrulename{Eq\_Scl\_SupNat}}{}%
}}

\newcommand{\ottdefnEqXXscequiv}[1]{\begin{ottdefnblock}[#1]{$\alpha  \sim  \alpha'$}{\ottcom{$\alpha$ is equal to $\alpha'$}}
\ottusedrule{\ottdruleEqXXSclXXSupBin{}}
\ottusedrule{\ottdruleEqXXSclXXSupNat{}}
\end{ottdefnblock}}

%% defn expequiv

\newcommand{\ottdefnEqXXexpequiv}[1]{\begin{ottdefnblock}[#1]{$\Gamma  \vdash  \ottnt{e}  \sim  \ottnt{e'}$}{\ottcom{$\ottnt{e}$ is equal to $\ottnt{e'}$}}
\end{ottdefnblock}}

%% defn stequiv
\newcommand{\ottdruleEqXXStgXXSupStat}[1]{\ottdrule[#1]{%
}{
  \stat   \lor  \mu   \sim  \mu}{%
{\ottdrulename{Eq\_Stg\_SupStat}}{}%
}}


\newcommand{\ottdruleEqXXStgXXSupDyn}[1]{\ottdrule[#1]{%
}{
  \dyn   \lor  \mu   \sim   \dyn }{%
{\ottdrulename{Eq\_Stg\_SupDyn}}{}%
}}


\newcommand{\ottdruleEqXXStgXXInfStat}[1]{\ottdrule[#1]{%
}{
  \stat   \land  \mu   \sim   \stat }{%
{\ottdrulename{Eq\_Stg\_InfStat}}{}%
}}


\newcommand{\ottdruleEqXXStgXXInfDyn}[1]{\ottdrule[#1]{%
}{
  \dyn   \land  \mu   \sim  \mu}{%
{\ottdrulename{Eq\_Stg\_InfDyn}}{}%
}}

\newcommand{\ottdefnEqXXstequiv}[1]{\begin{ottdefnblock}[#1]{$\mu  \sim  \mu'$}{\ottcom{$\mu$ is equal to $\mu'$}}
\ottusedrule{\ottdruleEqXXStgXXSupStat{}}
\ottusedrule{\ottdruleEqXXStgXXSupDyn{}}
\ottusedrule{\ottdruleEqXXStgXXInfStat{}}
\ottusedrule{\ottdruleEqXXStgXXInfDyn{}}
\end{ottdefnblock}}

%% defn tequiv
\newcommand{\ottdruleEqXXTyXXSupArr}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash   \ottnt{T_{{\mathrm{1}}}}  \land  \ottnt{T_{{\mathrm{2}}}}   \sim  \ottnt{T}  \hspace{1.5em}  \Gamma  \vdash   \ottnt{U_{{\mathrm{1}}}}  \lor  \ottnt{U_{{\mathrm{2}}}}   \sim  \ottnt{U} }%
}{
\Gamma  \vdash    (T_1 \times \cdots \times T_n)   \lor   (T_1 \times \cdots \times T_n)    \sim   (T_1 \times \cdots \times T_n) }{%
{\ottdrulename{Eq\_Ty\_SupArr}}{}%
}}


\newcommand{\ottdruleEqXXTyXXInfArr}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash   \ottnt{T_{{\mathrm{1}}}}  \lor  \ottnt{T_{{\mathrm{2}}}}   \sim  \ottnt{T}  \hspace{1.5em}  \Gamma  \vdash   \ottnt{U_{{\mathrm{1}}}}  \land  \ottnt{U_{{\mathrm{2}}}}   \sim  \ottnt{U} }%
}{
\Gamma  \vdash    (T_1 \times \cdots \times T_n)   \land   (T_1 \times \cdots \times T_n)    \sim  \ottnt{T}  \to  \ottnt{U}}{%
{\ottdrulename{Eq\_Ty\_InfArr}}{}%
}}


\newcommand{\ottdruleEqXXTyXXSupScl}[1]{\ottdrule[#1]{%
\ottpremise{  \mu_{{\mathrm{1}}}  \lor  \mu_{{\mathrm{2}}}   \sim  \mu  \hspace{1.5em}   \alpha_{{\mathrm{1}}}  \lor  \alpha_{{\mathrm{2}}}   \sim  \alpha }%
}{
\Gamma  \vdash    \Scalar{ \mu_{{\mathrm{1}}} }{ \alpha_{{\mathrm{1}}} }   \lor   \Scalar{ \mu_{{\mathrm{2}}} }{ \alpha_{{\mathrm{2}}} }    \sim   \Scalar{ \mu }{ \alpha } }{%
{\ottdrulename{Eq\_Ty\_SupScl}}{}%
}}


\newcommand{\ottdruleEqXXTyXXInfScl}[1]{\ottdrule[#1]{%
\ottpremise{  \mu_{{\mathrm{1}}}  \land  \mu_{{\mathrm{2}}}   \sim  \mu  \hspace{1.5em}   \alpha_{{\mathrm{1}}}  \land  \alpha_{{\mathrm{2}}}   \sim  \alpha }%
}{
\Gamma  \vdash    \Scalar{ \mu_{{\mathrm{1}}} }{ \alpha_{{\mathrm{1}}} }   \land   \Scalar{ \mu_{{\mathrm{2}}} }{ \alpha_{{\mathrm{2}}} }    \sim   \Scalar{ \mu }{ \alpha } }{%
{\ottdrulename{Eq\_Ty\_InfScl}}{}%
}}


\newcommand{\ottdruleEqXXTyXXSupSclRng}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash  \ottnt{e}  \checks   \Scalar{  \stat  }{  \mathbb{N}  }   \hspace{1.5em}    \mathbb{N}   \lor  \alpha   \sim  \alpha' }%
}{
\Gamma  \vdash    \Scalar{ \mu }{ \alpha }   \lor   \RangeNat{ \ottnt{e} }    \sim   \Scalar{ \mu }{ \alpha' } }{%
{\ottdrulename{Eq\_Ty\_SupSclRng}}{}%
}}


\newcommand{\ottdruleEqXXTyXXInfSclRng}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash  \ottnt{e}  \checks   \Scalar{  \stat  }{  \mathbb{N}  }   \hspace{1.5em}    \mathbb{N}   \land  \alpha   \sim  \alpha' }%
}{
\Gamma  \vdash    \Scalar{ \mu }{ \alpha }   \land   \RangeNat{ \ottnt{e} }    \sim   \Scalar{  \stat  }{ \alpha' } }{%
{\ottdrulename{Eq\_Ty\_InfSclRng}}{}%
}}


\newcommand{\ottdruleEqXXTyXXSupArray}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash  \delta_{\ottmv{i}}  \sim   \RangeNat{ \ottnt{e_{\ottmv{i}}} }   \hspace{1.5em}  \Gamma  \vdash  \delta'_{\ottmv{i}}  \sim   \RangeNat{ \ottnt{e'_{\ottmv{i}}} }  }%
\ottpremise{ \Gamma  \vdash  \ottnt{e_{\ottmv{i}}}  \sim  \ottnt{e'_{\ottmv{i}}}  \hspace{1.5em}  \Gamma  \vdash   \ottnt{T_{{\mathrm{1}}}}  \lor  \ottnt{T_{{\mathrm{2}}}}   \sim  \ottnt{T} }%
}{
\Gamma  \vdash    \ottnt{T_{{\mathrm{1}}}} ^{ \plural{\delta} }   \lor   \ottnt{T_{{\mathrm{2}}}} ^{ \plural{\delta}' }    \sim   \ottnt{T} ^{ \plural{\delta}_{{\mathrm{1}}} } }{%
{\ottdrulename{Eq\_Ty\_SupArray}}{}%
}}


\newcommand{\ottdruleEqXXTyXXInfArray}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash  \delta_{\ottmv{i}}  \sim   \RangeNat{ \ottnt{e_{\ottmv{i}}} }   \hspace{1.5em}  \Gamma  \vdash  \delta'_{\ottmv{i}}  \sim   \RangeNat{ \ottnt{e'_{\ottmv{i}}} }  }%
\ottpremise{ \Gamma  \vdash  \ottnt{e_{\ottmv{i}}}  \sim  \ottnt{e'_{\ottmv{i}}}  \hspace{1.5em}  \Gamma  \vdash   \ottnt{T_{{\mathrm{1}}}}  \land  \ottnt{T_{{\mathrm{2}}}}   \sim  \ottnt{T} }%
}{
\Gamma  \vdash    \ottnt{T_{{\mathrm{1}}}} ^{ \plural{\delta} }   \land   \ottnt{T_{{\mathrm{2}}}} ^{ \plural{\delta}' }    \sim   \ottnt{T} ^{ \plural{\delta}_{{\mathrm{1}}} } }{%
{\ottdrulename{Eq\_Ty\_InfArray}}{}%
}}


\newcommand{\ottdruleEqXXTyXXSupTDict}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash   \ottnt{K_{{\mathrm{1}}}}  \land  \ottnt{K_{{\mathrm{2}}}}   \sim  \ottnt{K}  \hspace{1.5em}  \Gamma  \vdash   \ottnt{T_{{\mathrm{1}}}}  \lor  \ottnt{T_{{\mathrm{2}}}}   \sim  \ottnt{T} }%
}{
\Gamma  \vdash    \TotalDict{ \ottnt{K_{{\mathrm{1}}}} }{ \ottnt{T_{{\mathrm{1}}}} }   \lor   \TotalDict{ \ottnt{K_{{\mathrm{2}}}} }{ \ottnt{T_{{\mathrm{2}}}} }    \sim   \TotalDict{ \ottnt{K} }{ \ottnt{T} } }{%
{\ottdrulename{Eq\_Ty\_SupTDict}}{}%
}}


\newcommand{\ottdruleEqXXTyXXSupPDict}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash   \ottnt{K_{{\mathrm{1}}}}  \land  \ottnt{K_{{\mathrm{2}}}}   \sim  \ottnt{K}  \hspace{1.5em}  \Gamma  \vdash   \ottnt{T_{{\mathrm{1}}}}  \lor  \ottnt{T_{{\mathrm{2}}}}   \sim  \ottnt{T} }%
}{
\Gamma  \vdash    \PartialDict{ \ottnt{K_{{\mathrm{1}}}} }{ \ottnt{T_{{\mathrm{1}}}} }   \lor   \PartialDict{ \ottnt{K_{{\mathrm{2}}}} }{ \ottnt{T_{{\mathrm{2}}}} }    \sim   \PartialDict{ \ottnt{K} }{ \ottnt{T} } }{%
{\ottdrulename{Eq\_Ty\_SupPDict}}{}%
}}

\newcommand{\ottdefnEqXXtequiv}[1]{\begin{ottdefnblock}[#1]{$\Gamma  \vdash  T  \sim  T'$}{\ottcom{$T$ is equal to $T'$}}
\ottusedrule{\ottdruleEqXXTyXXSupArr{}}
\ottusedrule{\ottdruleEqXXTyXXInfArr{}}
\ottusedrule{\ottdruleEqXXTyXXSupScl{}}
\ottusedrule{\ottdruleEqXXTyXXInfScl{}}
\ottusedrule{\ottdruleEqXXTyXXSupSclRng{}}
\ottusedrule{\ottdruleEqXXTyXXInfSclRng{}}
\ottusedrule{\ottdruleEqXXTyXXSupArray{}}
\ottusedrule{\ottdruleEqXXTyXXInfArray{}}
\ottusedrule{\ottdruleEqXXTyXXSupTDict{}}
\ottusedrule{\ottdruleEqXXTyXXSupPDict{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsEquality}{
\ottdefnEqXXdimeqv{}\ottdefnEqXXscequiv{}\ottdefnEqXXexpequiv{}\ottdefnEqXXstequiv{}\ottdefnEqXXtequiv{}}

% defns Subtyping
%% defn subtype
\newcommand{\ottdruleSubXXSup}[1]{\ottdrule[#1]{%
\ottpremise{\Gamma  \vdash   \ottnt{T}  \lor  \ottnt{T'}   \sim  \ottnt{T}}%
}{
\Gamma  \vdash  \ottnt{T}  \preccurlyeq  \ottnt{T'}}{%
{\ottdrulename{Sub\_Sup}}{}%
}}

\newcommand{\ottdefnsubtype}[1]{\begin{ottdefnblock}[#1]{$\Gamma  \vdash  \ottnt{T}  \preccurlyeq  \ottnt{T'}$}{\ottcom{$\ottnt{T}$ is a subtype of $\ottnt{T'}$}}
\ottusedrule{\ottdruleSubXXSup{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsSubtyping}{
\ottdefnsubtype{}}

% defns Formation
%% defn catlab

\newcommand{\ottdefnFXXcatlab}[1]{\begin{ottdefnblock}[#1]{$ \ell \ \mathbf{label} $}{\ottcom{$\ell$ is a category label}}
\end{ottdefnblock}}

%% defn freshvar

\newcommand{\ottdefnFXXfreshvar}[1]{\begin{ottdefnblock}[#1]{$ \mathit{a} \ \textbf{fresh} $}{\ottcom{$\mathit{a}$ is a fresh variable}}
\end{ottdefnblock}}

%% defn tkey
\newcommand{\ottdruleFXXTKXXRngNat}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash   \RangeNat{ \ottnt{e} }  \ \mathbf{type} }%
}{
 \Gamma  \vdash   \RangeNat{ \ottnt{e} }  \ \mathbf{total\ key} }{%
{\ottdrulename{F\_TK\_RngNat}}{}%
}}


\newcommand{\ottdruleFXXTKXXCatLab}[1]{\ottdrule[#1]{%
\ottpremise{ \ell \ \mathbf{label} }%
}{
 \Gamma  \vdash   \CatLab{ \ell }  \ \mathbf{total\ key} }{%
{\ottdrulename{F\_TK\_CatLab}}{}%
}}


\newcommand{\ottdruleFXXTKXXTupleKey}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash  \ottnt{K_{\ottmv{i}}} \ \mathbf{total\ key} }%
}{
 \Gamma  \vdash   (T_1 \times \cdots \times T_n)  \ \mathbf{total\ key} }{%
{\ottdrulename{F\_TK\_TupleKey}}{}%
}}


\newcommand{\ottdruleFXXTKXXTKeys}[1]{\ottdrule[#1]{%
\ottpremise{\Gamma  \shortmid   \emptyset   \vdash  \ottnt{e}  \infers   \TotalDict{ \ottnt{K} }{ \ottnt{T} } }%
}{
 \Gamma  \vdash   \PromotedSet{  \textsf{keys}   \ottsym{(}  \ottnt{e}  \ottsym{)} }  \ \mathbf{total\ key} }{%
{\ottdrulename{F\_TK\_TKeys}}{}%
}}


\newcommand{\ottdruleFXXTKXXPKeys}[1]{\ottdrule[#1]{%
\ottpremise{\Gamma  \shortmid   \emptyset   \vdash  \ottnt{e}  \infers   \PartialDict{ \ottnt{K} }{ \ottnt{T} } }%
}{
 \Gamma  \vdash   \PromotedSet{  \textsf{keys}   \ottsym{(}  \ottnt{e}  \ottsym{)} }  \ \mathbf{total\ key} }{%
{\ottdrulename{F\_TK\_PKeys}}{}%
}}

\newcommand{\ottdefnFXXtkey}[1]{\begin{ottdefnblock}[#1]{$ \Gamma  \vdash  \ottnt{T} \ \mathbf{total\ key} $}{\ottcom{$\ottnt{T}$ can be a key of total dictionary}}
\ottusedrule{\ottdruleFXXTKXXRngNat{}}
\ottusedrule{\ottdruleFXXTKXXCatLab{}}
\ottusedrule{\ottdruleFXXTKXXTupleKey{}}
\ottusedrule{\ottdruleFXXTKXXTKeys{}}
\ottusedrule{\ottdruleFXXTKXXPKeys{}}
\end{ottdefnblock}}

%% defn pkey
\newcommand{\ottdruleFXXPKXXInt}[1]{\ottdrule[#1]{%
\ottpremise{\Gamma  \vdash  \ottnt{T}  \preccurlyeq   \Scalar{  \stat  }{  \mathbb{Z}  } }%
}{
 \Gamma  \vdash  \ottnt{T} \ \mathbf{partial\ key} }{%
{\ottdrulename{F\_PK\_Int}}{}%
}}


\newcommand{\ottdruleFXXPKXXCatLab}[1]{\ottdrule[#1]{%
\ottpremise{ \ell \ \mathbf{label} }%
}{
 \Gamma  \vdash   \CatLab{ \ell }  \ \mathbf{partial\ key} }{%
{\ottdrulename{F\_PK\_CatLab}}{}%
}}


\newcommand{\ottdruleFXXPKXXStr}[1]{\ottdrule[#1]{%
}{
 \Gamma  \vdash  \ottkw{String} \ \mathbf{partial\ key} }{%
{\ottdrulename{F\_PK\_Str}}{}%
}}


\newcommand{\ottdruleFXXPKXXTupleKey}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash  \ottnt{K_{\ottmv{i}}} \ \mathbf{partial\ key} }%
}{
 \Gamma  \vdash   (T_1 \times \cdots \times T_n)  \ \mathbf{partial\ key} }{%
{\ottdrulename{F\_PK\_TupleKey}}{}%
}}

\newcommand{\ottdefnFXXpkey}[1]{\begin{ottdefnblock}[#1]{$ \Gamma  \vdash  \ottnt{T} \ \mathbf{partial\ key} $}{\ottcom{$\ottnt{T}$ can be a key of partial dictionary}}
\ottusedrule{\ottdruleFXXPKXXInt{}}
\ottusedrule{\ottdruleFXXPKXXCatLab{}}
\ottusedrule{\ottdruleFXXPKXXStr{}}
\ottusedrule{\ottdruleFXXPKXXTupleKey{}}
\end{ottdefnblock}}

%% defn type
\newcommand{\ottdruleFXXTXXRangeNat}[1]{\ottdrule[#1]{%
\ottpremise{\Gamma  \vdash  \ottnt{e}  \checks   \Scalar{  \stat  }{  \mathbb{N}  } }%
}{
 \Gamma  \vdash   \RangeNat{ \ottnt{e} }  \ \mathbf{type} }{%
{\ottdrulename{F\_T\_RangeNat}}{}%
}}


\newcommand{\ottdruleFXXTXXCatLab}[1]{\ottdrule[#1]{%
\ottpremise{ \ell \ \mathbf{label} }%
}{
 \Gamma  \vdash   \CatLab{ \ell }  \ \mathbf{type} }{%
{\ottdrulename{F\_T\_CatLab}}{}%
}}


\newcommand{\ottdruleFXXTXXTDict}[1]{\ottdrule[#1]{%
\ottpremise{  \Gamma  \vdash  \ottnt{K} \ \mathbf{total\ key}   \hspace{1.5em}   \Gamma  \vdash  \ottnt{T} \ \mathbf{type}  }%
}{
 \Gamma  \vdash   \TotalDict{ \ottnt{K} }{ \ottnt{T} }  \ \mathbf{type} }{%
{\ottdrulename{F\_T\_TDict}}{}%
}}


\newcommand{\ottdruleFXXTXXPDict}[1]{\ottdrule[#1]{%
\ottpremise{  \Gamma  \vdash  \ottnt{K} \ \mathbf{partial\ key}   \hspace{1.5em}   \Gamma  \vdash  \ottnt{T} \ \mathbf{type}  }%
}{
 \Gamma  \vdash   \PartialDict{ \ottnt{K} }{ \ottnt{T} }  \ \mathbf{type} }{%
{\ottdrulename{F\_T\_PDict}}{}%
}}

\newcommand{\ottdefnFXXtype}[1]{\begin{ottdefnblock}[#1]{$ \Gamma  \vdash  \ottnt{T} \ \mathbf{type} $}{\ottcom{$\ottnt{T}$ is a type}}
\ottusedrule{\ottdruleFXXTXXRangeNat{}}
\ottusedrule{\ottdruleFXXTXXCatLab{}}
\ottusedrule{\ottdruleFXXTXXTDict{}}
\ottusedrule{\ottdruleFXXTXXPDict{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsFormation}{
\ottdefnFXXcatlab{}\ottdefnFXXfreshvar{}\ottdefnFXXtkey{}\ottdefnFXXpkey{}\ottdefnFXXtype{}}

% defns Typing
%% defn infers
\newcommand{\ottdruleTXXIXXAbs}[1]{\ottdrule[#1]{%
\ottpremise{\Gamma  \vdash  \ottnt{p}  \checks  \ottnt{T_{{\mathrm{1}}}}  \infers  \ottnt{D}}%
\ottpremise{ D \left\{  \ottnt{p}  :  \ottnt{T_{{\mathrm{1}}}}  \right\} ,  \Gamma   \shortmid  \Psi  \vdash  \ottnt{e}  \infers  \ottnt{T_{{\mathrm{2}}}}}%
}{
\Gamma  \shortmid   \Psi  ,  \ottnt{T_{{\mathrm{1}}}}   \vdash   \lambda  \ottnt{p} \ldotp  \ottnt{e}   \infers  \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}}{%
{\ottdrulename{T\_I\_Abs}}{}%
}}


\newcommand{\ottdruleTXXIXXApp}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \shortmid   \emptyset   \vdash  \ottnt{e_{{\mathrm{2}}}}  \infers  \ottnt{T_{{\mathrm{1}}}}  \hspace{1.5em}  \Gamma  \shortmid   \Psi  ,  \ottnt{T_{{\mathrm{1}}}}   \vdash  \ottnt{e_{{\mathrm{1}}}}  \infers  \ottnt{T_{{\mathrm{2}}}} }%
}{
\Gamma  \shortmid  \Psi  \vdash  \ottnt{e_{{\mathrm{1}}}} \, \ottnt{e_{{\mathrm{2}}}}  \infers  \ottnt{T}}{%
{\ottdrulename{T\_I\_App}}{}%
}}


\newcommand{\ottdruleTXXIXXIterCat}[1]{\ottdrule[#1]{%
\ottpremise{ \ell \ \mathbf{label} }%
}{
\Gamma  \shortmid   \emptyset   \vdash   \IterCat{l}   \ottsym{(}  \,  \ottsym{)}  \infers   \SetOf{  \CatLab{ \ell }  } }{%
{\ottdrulename{T\_I\_IterCat}}{}%
}}


\newcommand{\ottdruleTXXIXXList}[1]{\ottdrule[#1]{%
\ottpremise{\Gamma  \shortmid   \emptyset   \vdash  \ottnt{e_{\ottmv{i}}}  \infers  \ottnt{T_{\ottmv{i}}}}%
\ottpremise{\Gamma  \vdash   \ottnt{T_{{\mathrm{1}}}}  \lor \ldots \lor  \ottnt{T_{\ottmv{n}}}   \sim  \ottnt{T}}%
}{
\Gamma  \shortmid   \emptyset   \vdash  \ottsym{[}  \ottnt{e_{{\mathrm{1}}}}  \ottsym{,} \, .. \, \ottsym{,}  \ottnt{e_{\ottmv{n}}}  \ottsym{]}  \infers   \ottnt{T} ^{   \RangeNat{ \ottmv{n} }   } }{%
{\ottdrulename{T\_I\_List}}{}%
}}


\newcommand{\ottdruleTXXIXXUnionSet}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \shortmid   \emptyset   \vdash  \ottnt{e_{\ottmv{i}}}  \infers   \SetOf{ \ottnt{T_{\ottmv{i}}} }   \hspace{1.5em}  \Gamma  \vdash   \ottnt{T_{{\mathrm{1}}}}  \lor  \ottnt{T_{{\mathrm{2}}}}   \sim  \ottnt{T} }%
}{
\Gamma  \shortmid   \emptyset   \vdash   \textsf{union}   \ottsym{(}  \ottnt{e_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{e_{{\mathrm{2}}}}  \ottsym{)}  \infers   \SetOf{ \ottnt{T} } }{%
{\ottdrulename{T\_I\_UnionSet}}{}%
}}


\newcommand{\ottdruleTXXIXXIntersectSet}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \shortmid   \emptyset   \vdash  \ottnt{e_{\ottmv{i}}}  \infers   \SetOf{ \ottnt{T_{\ottmv{i}}} }   \hspace{1.5em}  \Gamma  \vdash   \ottnt{T_{{\mathrm{1}}}}  \land  \ottnt{T_{{\mathrm{2}}}}   \sim  \ottnt{T} }%
}{
\Gamma  \shortmid   \emptyset   \vdash   \textsf{intersect}   \ottsym{(}  \ottnt{e_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{e_{{\mathrm{2}}}}  \ottsym{)}  \infers   \SetOf{ \ottnt{T} } }{%
{\ottdrulename{T\_I\_IntersectSet}}{}%
}}


\newcommand{\ottdruleTXXIXXSubsFull}[1]{\ottdrule[#1]{%
\ottpremise{\Gamma  \shortmid   \emptyset   \vdash  \ottnt{e}  \infers   \ottnt{T} ^{  \delta_{{\mathrm{1}}}  , \ldots ,  \delta_{\ottmv{n}}  } }%
\ottpremise{\Gamma  \vdash  \ottnt{e_{\ottmv{i}}}  \checks   \Scalar{  \stat  }{  \mathbb{N}  } }%
}{
\Gamma  \shortmid   \emptyset   \vdash  \ottnt{e} \, \ottsym{[}  \ottnt{e_{{\mathrm{1}}}}  \ottsym{,} \, .. \, \ottsym{,}  \ottnt{e_{\ottmv{n}}}  \ottsym{]}  \infers  \ottnt{T}}{%
{\ottdrulename{T\_I\_SubsFull}}{}%
}}


\newcommand{\ottdruleTXXIXXSubsSub}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \shortmid   \emptyset   \vdash  \ottnt{e}  \infers   \ottnt{T} ^{  \delta_{{\mathrm{1}}}  , \ldots ,  \delta_{\ottmv{n}}  }   \hspace{1.5em}   \ottmv{k}  <  \ottmv{n}  }%
\ottpremise{\Gamma  \vdash  \ottnt{e_{\ottmv{i}}}  \checks   \Scalar{  \stat  }{  \mathbb{N}  } }%
}{
\Gamma  \shortmid   \emptyset   \vdash  \ottnt{e} \, \ottsym{[}  \ottnt{e_{{\mathrm{1}}}}  \ottsym{,} \, .. \, \ottsym{,}  \ottnt{e_{\ottmv{k}}}  \ottsym{]}  \infers   \ottnt{T} ^{  \delta_{\ottmv{k + 1}}  , \ldots ,  \delta_{\ottmv{n}}  } }{%
{\ottdrulename{T\_I\_SubsSub}}{}%
}}


\newcommand{\ottdruleTXXIXXLookupTotal}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \shortmid   \emptyset   \vdash  \ottnt{e}  \infers   \TotalDict{ \ottnt{K} }{ \ottnt{T} }   \hspace{1.5em}  \Gamma  \vdash  \ottnt{e'}  \checks  \ottnt{K} }%
}{
\Gamma  \shortmid   \emptyset   \vdash  \ottnt{e} \, \ottsym{[}  \ottnt{e'}  \ottsym{]}  \infers  \ottnt{T}}{%
{\ottdrulename{T\_I\_LookupTotal}}{}%
}}


\newcommand{\ottdruleTXXIXXLookupPartial}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \shortmid   \emptyset   \vdash  \ottnt{e}  \infers   \PartialDict{ \ottnt{K} }{ \ottnt{T} }   \hspace{1.5em}  \Gamma  \vdash  \ottnt{e'}  \checks   \PromotedSet{  \textsf{keys}   \ottsym{(}  \ottnt{e}  \ottsym{)} }  }%
}{
\Gamma  \shortmid   \emptyset   \vdash  \ottnt{e} \, \ottsym{[}  \ottnt{e'}  \ottsym{]}  \infers  \ottnt{T}}{%
{\ottdrulename{T\_I\_LookupPartial}}{}%
}}


\newcommand{\ottdruleTXXIXXDiv}[1]{\ottdrule[#1]{%
\ottpremise{  \Gamma  \shortmid   \emptyset   \vdash  \ottnt{e}  \infers   \Scalar{ \mu_{{\mathrm{1}}} }{ \alpha }   \hspace{1.5em}  \Gamma  \shortmid   \emptyset   \vdash  \ottnt{e'}  \infers   \Scalar{ \mu_{{\mathrm{2}}} }{ \alpha }    \hspace{1.5em}   \mu_{{\mathrm{1}}}  \lor  \mu_{{\mathrm{2}}}   \sim  \mu' }%
}{
\Gamma  \shortmid   \emptyset   \vdash   \textsf{div}   \ottsym{(}  \ottnt{e}  \ottsym{,}  \ottnt{e'}  \ottsym{)}  \infers   \Scalar{ \mu' }{  \mathbb{R}  } }{%
{\ottdrulename{T\_I\_Div}}{}%
}}

\newcommand{\ottdefnTXXinfers}[1]{\begin{ottdefnblock}[#1]{$\Gamma  \shortmid  \Psi  \vdash  \ottnt{e}  \infers  \ottnt{T}$}{\ottcom{$\ottnt{e}$ is inferred to have type $\ottnt{T}$ in context $\Gamma$}}
\ottusedrule{\ottdruleTXXIXXAbs{}}
\ottusedrule{\ottdruleTXXIXXApp{}}
\ottusedrule{\ottdruleTXXIXXIterCat{}}
\ottusedrule{\ottdruleTXXIXXList{}}
\ottusedrule{\ottdruleTXXIXXUnionSet{}}
\ottusedrule{\ottdruleTXXIXXIntersectSet{}}
\ottusedrule{\ottdruleTXXIXXSubsFull{}}
\ottusedrule{\ottdruleTXXIXXSubsSub{}}
\ottusedrule{\ottdruleTXXIXXLookupTotal{}}
\ottusedrule{\ottdruleTXXIXXLookupPartial{}}
\ottusedrule{\ottdruleTXXIXXDiv{}}
\end{ottdefnblock}}

%% defn checks
\newcommand{\ottdruleTXXCXXAbs}[1]{\ottdrule[#1]{%
\ottpremise{\Gamma  \vdash  \ottnt{p}  \checks  \ottnt{T_{{\mathrm{1}}}}  \infers  \ottnt{D}}%
\ottpremise{ D \left\{  \ottnt{p}  :  \ottnt{T_{{\mathrm{1}}}}  \right\} ,  \Gamma   \vdash  \ottnt{e}  \checks  \ottnt{T_{{\mathrm{2}}}}}%
}{
\Gamma  \vdash   \lambda  \ottnt{p} \ldotp  \ottnt{e}   \checks  \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}}{%
{\ottdrulename{T\_C\_Abs}}{}%
}}


\newcommand{\ottdruleTXXCXXChangeDir}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \shortmid   \emptyset   \vdash  \ottnt{e}  \infers  \ottnt{T'}  \hspace{1.5em}  \Gamma  \vdash  \ottnt{T'}  \preccurlyeq  \ottnt{T} }%
}{
\Gamma  \vdash  \ottnt{e}  \checks  \ottnt{T}}{%
{\ottdrulename{T\_C\_ChangeDir}}{}%
}}


\newcommand{\ottdruleTXXCXXKeysApprox}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \shortmid   \emptyset   \vdash  \ottnt{e}  \infers  \ottnt{T}  \hspace{1.5em}  \Gamma  \vdash  \ottnt{e}  \checks   \SetOf{ \ottnt{T} }  }%
}{
\Gamma  \vdash  \ottnt{e}  \checks   \PromotedSet{  \textsf{keys}   \ottsym{(}  \ottnt{e'}  \ottsym{)} } }{%
{\ottdrulename{T\_C\_KeysApprox}}{}%
}}

\newcommand{\ottdefnTXXchecks}[1]{\begin{ottdefnblock}[#1]{$\Gamma  \vdash  \ottnt{e}  \checks  \ottnt{T}$}{\ottcom{$\ottnt{e}$ is inferred to have type $\ottnt{T}$ in context $\Gamma$}}
\ottusedrule{\ottdruleTXXCXXAbs{}}
\ottusedrule{\ottdruleTXXCXXChangeDir{}}
\ottusedrule{\ottdruleTXXCXXKeysApprox{}}
\end{ottdefnblock}}

%% defn destructs
\newcommand{\ottdruleTXXPXXVar}[1]{\ottdrule[#1]{%
}{
\Gamma  \vdash  x_{\ottmv{i}}  \checks  \ottnt{T}  \infers   \left(x_{ \ottmv{i} } :  \ottnt{T}  \right) }{%
{\ottdrulename{T\_P\_Var}}{}%
}}


\newcommand{\ottdruleTXXPXXTuple}[1]{\ottdrule[#1]{%
\ottpremise{\Gamma  \vdash  \ottnt{p_{\ottmv{i}}}  \checks  \ottnt{T_{\ottmv{i}}}  \infers  \ottnt{D_{\ottmv{i}}}}%
}{
\Gamma  \vdash  \ottsym{(}  \ottnt{p_{{\mathrm{1}}}}  \ottsym{,} \, .. \, \ottsym{,}  \ottnt{p_{\ottmv{n}}}  \ottsym{)}  \checks   (T_1 \times \cdots \times T_n)   \infers   \mathbf{tuple}_{D_1, \ldots, D_n} }{%
{\ottdrulename{T\_P\_Tuple}}{}%
}}


\newcommand{\ottdruleTXXPXXArray}[1]{\ottdrule[#1]{%
\ottpremise{\Gamma  \vdash  \ottnt{p_{\ottmv{i}}}  \checks   \ottnt{T} ^{ \plural{\delta} }   \infers  \ottnt{D_{\ottmv{i}}}}%
}{
\Gamma  \vdash  \ottsym{(}  \ottnt{p_{{\mathrm{1}}}}  \ottsym{,} \, .. \, \ottsym{,}  \ottnt{p_{\ottmv{n}}}  \ottsym{)}  \checks   \ottnt{T} ^{   \RangeNat{ \ottmv{n} }   ,  \plural{\delta}  }   \infers   \mathbf{Array}_{D_1, \ldots, D_n} }{%
{\ottdrulename{T\_P\_Array}}{}%
}}

\newcommand{\ottdefnTXXdestructs}[1]{\begin{ottdefnblock}[#1]{$\Gamma  \vdash  \ottnt{p}  \checks  \ottnt{T}  \infers  \ottnt{D}$}{\ottcom{checks pattern $\ottnt{p}$ against type $\ottnt{T}$, producing destructors $\ottnt{D}$}}
\ottusedrule{\ottdruleTXXPXXVar{}}
\ottusedrule{\ottdruleTXXPXXTuple{}}
\ottusedrule{\ottdruleTXXPXXArray{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsTyping}{
\ottdefnTXXinfers{}\ottdefnTXXchecks{}\ottdefnTXXdestructs{}}

% defns Desugar
%% defn desugar_comp_stmts
\newcommand{\ottdruleDXXCompXXForIn}[1]{\ottdrule[#1]{%
}{
 \CompStmtDesugarTo{  \textbf{for }  \ottnt{p}  \ \textbf{in }  \ottnt{e}  }{ \ottnt{p} }{ \ottnt{e} } }{%
{\ottdrulename{D\_Comp\_ForIn}}{}%
}}


\newcommand{\ottdruleDXXCompXXForInCons}[1]{\ottdrule[#1]{%
\ottpremise{ \CompStmtDesugarTo{ \plural{C} }{ \ottnt{p_{{\mathrm{0}}}} }{ \ottnt{e'} } }%
}{
 \CompStmtDesugarTo{  \plural{C}  ;\    \textbf{for }  \ottnt{p}  \ \textbf{in }  \ottnt{e}   }{ \ottsym{(}  \ottnt{p_{{\mathrm{0}}}}  \ottsym{,}  \ottnt{p}  \ottsym{)} }{  \textsf{flat\_map}   \ottsym{(}   \lambda  \ottnt{p_{{\mathrm{0}}}} \ldotp   \textsf{map}   \ottsym{(}   \lambda  \ottnt{p} \ldotp  \ottsym{(}  \ottnt{p_{{\mathrm{0}}}}  \ottsym{,}  \ottnt{p}  \ottsym{)}   \ottsym{,}  \ottnt{e}  \ottsym{)}   \ottsym{,}  \ottnt{e'}  \ottsym{)} } }{%
{\ottdrulename{D\_Comp\_ForInCons}}{}%
}}


\newcommand{\ottdruleDXXCompXXIfCons}[1]{\ottdrule[#1]{%
\ottpremise{ \CompStmtDesugarTo{ \plural{C} }{ \ottnt{p} }{ \ottnt{e'} } }%
}{
 \CompStmtDesugarTo{  \plural{C}  ;\    \textbf{if }  \ottnt{e}   }{ \ottnt{p} }{  \textsf{filter}   \ottsym{(}   \lambda  \ottnt{p} \ldotp  \ottnt{e}   \ottsym{,}  \ottnt{e'}  \ottsym{)} } }{%
{\ottdrulename{D\_Comp\_IfCons}}{}%
}}

\newcommand{\ottdefnDXXdesugarXXcompXXstmts}[1]{\begin{ottdefnblock}[#1]{$ \CompStmtDesugarTo{ \plural{C} }{ \ottnt{p} }{ \ottnt{e} } $}{\ottcom{desugars comprehension statements $\plural{C}$ into expression $\ottnt{e}$ with continuation arguments $\ottnt{p}$}}
\ottusedrule{\ottdruleDXXCompXXForIn{}}
\ottusedrule{\ottdruleDXXCompXXForInCons{}}
\ottusedrule{\ottdruleDXXCompXXIfCons{}}
\end{ottdefnblock}}

%% defn desugar_comp
\newcommand{\ottdruleDXXCompXXListComp}[1]{\ottdrule[#1]{%
\ottpremise{ \CompStmtDesugarTo{ \plural{C} }{ \ottnt{p} }{ \ottnt{e'} } }%
}{
 [\  \ottnt{e}  \mid   \plural{C}  \ ]   \leadsto   \textsf{map}   \ottsym{(}   \lambda  \ottnt{p} \ldotp  \ottnt{e}   \ottsym{,}  \ottnt{e'}  \ottsym{)}}{%
{\ottdrulename{D\_Comp\_ListComp}}{}%
}}

\newcommand{\ottdefnDXXdesugarXXcomp}[1]{\begin{ottdefnblock}[#1]{$\ottnt{compr}  \leadsto  \ottnt{e}$}{\ottcom{desugars comprehension $\ottnt{compr}$ into expression $\ottnt{e}$}}
\ottusedrule{\ottdruleDXXCompXXListComp{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsDesugar}{
\ottdefnDXXdesugarXXcompXXstmts{}\ottdefnDXXdesugarXXcomp{}}

% defns Ensugar
%% defn ensugar_comp_stmts
\newcommand{\ottdruleESXXStmtsXXMap}[1]{\ottdrule[#1]{%
\ottpremise{  \plural{a} \ \textbf{fresh}   \hspace{1.5em}   \{\!| \   {}^{\setminus  \plural{a} }{ \ottnt{p'} }   \in  \ottnt{e'}  \ |\!\} =  \plural{\kappa}  }%
}{
 \{\!| \  \ottnt{p}  \in   \textsf{map}   \ottsym{(}   \lambda  \ottnt{p'} \ldotp  \ottnt{e}   \ottsym{,}  \ottnt{e'}  \ottsym{)}  \ |\!\} =   \plural{\kappa} ;\   \textbf{let }  \ottnt{p}  =   {}^{\setminus  \plural{a} }{ \ottnt{e} }    }{%
{\ottdrulename{ES\_Stmts\_Map}}{}%
}}


\newcommand{\ottdruleESXXStmtsXXFlatMap}[1]{\ottdrule[#1]{%
\ottpremise{ \plural{a} \ \textbf{fresh} }%
\ottpremise{  \{\!| \   {}^{\setminus  \plural{a} }{ \ottnt{p'} }   \in  \ottnt{e'}  \ |\!\} =  \plural{\kappa}   \hspace{1.5em}   \{\!| \  \ottnt{p}  \in   {}^{\setminus  \plural{a} }{ \ottnt{e} }   \ |\!\} =  \plural{\kappa}'  }%
}{
 \{\!| \  \ottnt{p}  \in   \textsf{flat\_map}   \ottsym{(}   \lambda  \ottnt{p'} \ldotp  \ottnt{e}   \ottsym{,}  \ottnt{e'}  \ottsym{)}  \ |\!\} =   \plural{\kappa} ;\  \plural{\kappa}'  }{%
{\ottdrulename{ES\_Stmts\_FlatMap}}{}%
}}


\newcommand{\ottdruleESXXStmtsXXFilter}[1]{\ottdrule[#1]{%
\ottpremise{  \plural{a} \ \textbf{fresh}   \hspace{1.5em}   \{\!| \   {}^{\setminus  \plural{a} }{ \ottnt{p'} }   \in  \ottnt{e'}  \ |\!\} =  \plural{\kappa}  }%
}{
 \{\!| \  \ottnt{p}  \in   \textsf{filter}   \ottsym{(}   \lambda  \ottnt{p'} \ldotp  \ottnt{e}   \ottsym{,}  \ottnt{e'}  \ottsym{)}  \ |\!\} =    \plural{\kappa} ;\   \textbf{if }   {}^{\setminus  \plural{a} }{ \ottnt{e} }    ;\   \textbf{let }  \ottnt{p}  =   {}^{\setminus  \plural{a} }{ \ottnt{p'} }    }{%
{\ottdrulename{ES\_Stmts\_Filter}}{}%
}}


\newcommand{\ottdruleESXXStmtsXXFallback}[1]{\ottdrule[#1]{%
}{
 \{\!| \  \ottnt{p}  \in  \ottnt{e}  \ |\!\} =   \textbf{for }  \ottnt{p}  \ \textbf{in }  \ottnt{e}  }{%
{\ottdrulename{ES\_Stmts\_Fallback}}{}%
}}

\newcommand{\ottdefnESXXensugarXXcompXXstmts}[1]{\begin{ottdefnblock}[#1]{$ \{\!| \  \ottnt{p}  \in  \ottnt{e}  \ |\!\} =  \plural{\kappa} $}{\ottcom{ensugars expression iterating over $\ottnt{e}$ as $\ottnt{p}$ into comprehension statements $\plural{\kappa}$}}
\ottusedrule{\ottdruleESXXStmtsXXMap{}}
\ottusedrule{\ottdruleESXXStmtsXXFlatMap{}}
\ottusedrule{\ottdruleESXXStmtsXXFilter{}}
\ottusedrule{\ottdruleESXXStmtsXXFallback{}}
\end{ottdefnblock}}

%% defn ensugar_listcomp
\newcommand{\ottdruleESXXCompXXMap}[1]{\ottdrule[#1]{%
\ottpremise{  \plural{a} \ \textbf{fresh}   \hspace{1.5em}   \{\!| \   {}^{\setminus  \plural{a} }{ \ottnt{p} }   \in  \ottnt{e'}  \ |\!\} =  \plural{\kappa}  }%
}{
 \llbracket   \textsf{map}   \ottsym{(}   \lambda  \ottnt{p} \ldotp  \ottnt{e}   \ottsym{,}  \ottnt{e'}  \ottsym{)}  \rrbracket =   [ \   {}^{\setminus  \plural{a} }{ \ottnt{e} }   \mid  \plural{\kappa}  \ ]  }{%
{\ottdrulename{ES\_Comp\_Map}}{}%
}}


\newcommand{\ottdruleESXXCompXXFlatMap}[1]{\ottdrule[#1]{%
\ottpremise{    \plural{a} \ \textbf{fresh}   \hspace{1.5em}   \mathit{b} \ \textbf{fresh}    \hspace{1.5em}   \{\!| \   {}^{\setminus  \plural{a} }{ \ottnt{p} }   \in  \ottnt{e'}  \ |\!\} =  \plural{\kappa}    \hspace{1.5em}   \{\!| \  \mathit{b}  \in   {}^{\setminus  \plural{a} }{ \ottnt{p} }   \ |\!\} =  \plural{\kappa}'  }%
}{
 \llbracket   \textsf{flat\_map}   \ottsym{(}   \lambda  \ottnt{p} \ldotp  \ottnt{e}   \ottsym{,}  \ottnt{e'}  \ottsym{)}  \rrbracket =   [ \  \mathit{b}  \mid   \plural{\kappa} ;\  \plural{\kappa}'   \ ]  }{%
{\ottdrulename{ES\_Comp\_FlatMap}}{}%
}}


\newcommand{\ottdruleESXXCompXXFilter}[1]{\ottdrule[#1]{%
\ottpremise{  \plural{a} \ \textbf{fresh}   \hspace{1.5em}   \llbracket  \ottnt{e'}  \rrbracket =   [ \  \ottnt{e_{{\mathrm{0}}}}  \mid  \plural{\kappa}  \ ]   }%
}{
 \llbracket   \textsf{filter}   \ottsym{(}   \lambda  \ottnt{p} \ldotp  \ottnt{e}   \ottsym{,}  \ottnt{e'}  \ottsym{)}  \rrbracket =   [ \  \ottnt{e_{{\mathrm{0}}}}  \mid    \plural{\kappa} ;\   \textbf{let }   {}^{\setminus  \plural{a} }{ \ottnt{p} }   =  \ottnt{e_{{\mathrm{0}}}}   ;\   \textbf{if }   {}^{\setminus  \plural{a} }{ \ottnt{e} }     \ ]  }{%
{\ottdrulename{ES\_Comp\_Filter}}{}%
}}

\newcommand{\ottdefnESXXensugarXXlistcomp}[1]{\begin{ottdefnblock}[#1]{$ \llbracket  \ottnt{e}  \rrbracket =  \ottnt{extended\_comprehension} $}{\ottcom{ensugars expression $\ottnt{e}$ into list comprehension $\ottnt{extended\_comprehension}$}}
\ottusedrule{\ottdruleESXXCompXXMap{}}
\ottusedrule{\ottdruleESXXCompXXFlatMap{}}
\ottusedrule{\ottdruleESXXCompXXFilter{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsEnsugar}{
\ottdefnESXXensugarXXcompXXstmts{}\ottdefnESXXensugarXXlistcomp{}}

\newcommand{\ottdefnss}{
\ottdefnsEquality
\ottdefnsSubtyping
\ottdefnsFormation
\ottdefnsTyping
\ottdefnsDesugar
\ottdefnsEnsugar
}

\newcommand{\ottall}{\ottmetavars\\[0pt]
\ottgrammar\\[5.0mm]
\ottdefnss}



==> value.ott.tex <==
% generated by Ott 0.34 from: ott/value.ott
\newcommand{\ottdrule}[4][]{{\displaystyle\frac{\begin{array}{l}#2\end{array}}{#3}\quad\ottdrulename{#4}}}
\newcommand{\ottusedrule}[1]{\[#1\]}
\newcommand{\ottpremise}[1]{ #1 \\}
\newenvironment{ottdefnblock}[3][]{ \framebox{\mbox{#2}} \quad #3 \\[0pt]}{}
\newenvironment{ottfundefnblock}[3][]{ \framebox{\mbox{#2}} \quad #3 \\[0pt]\begin{displaymath}\begin{array}{l}}{\end{array}\end{displaymath}}
\newcommand{\ottfunclause}[2]{ #1 \equiv #2 \\}
\newcommand{\ottnt}[1]{\mathit{#1}}
\newcommand{\ottmv}[1]{\mathit{#1}}
\newcommand{\ottkw}[1]{\mathbf{#1}}
\newcommand{\ottsym}[1]{#1}
\newcommand{\ottcom}[1]{\text{#1}}
\newcommand{\ottdrulename}[1]{\textsc{#1}}
\newcommand{\ottcomplu}[5]{\overline{#1}^{\,#2\in #3 #4 #5}}
\newcommand{\ottcompu}[3]{\overline{#1}^{\,#2<#3}}
\newcommand{\ottcomp}[2]{\overline{#1}^{\,#2}}
\newcommand{\ottgrammartabular}[1]{\begin{supertabular}{llcllllll}#1\end{supertabular}}
\newcommand{\ottmetavartabular}[1]{\begin{supertabular}{ll}#1\end{supertabular}}
\newcommand{\ottrulehead}[3]{$#1$ & & $#2$ & & & \multicolumn{2}{l}{#3}}
\newcommand{\ottprodline}[6]{& & $#1$ & $#2$ & $#3 #4$ & $#5$ & $#6$}
\newcommand{\ottfirstprodline}[6]{\ottprodline{#1}{#2}{#3}{#4}{#5}{#6}}
\newcommand{\ottlongprodline}[2]{& & $#1$ & \multicolumn{4}{l}{$#2$}}
\newcommand{\ottfirstlongprodline}[2]{\ottlongprodline{#1}{#2}}
\newcommand{\ottbindspecprodline}[6]{\ottprodline{#1}{#2}{#3}{#4}{#5}{#6}}
\newcommand{\ottprodnewline}{\\}
\newcommand{\ottinterrule}{\\[5.0mm]}
\newcommand{\ottafterlastrule}{\\}
\newcommand{\ottmetavars}{
\ottmetavartabular{
 $ \ottmv{fp} $ & \ottcom{floating-point number} \\
 $ \ottmv{index} ,\, \ottmv{i} ,\, \ottmv{j} ,\, \ottmv{k} ,\, \ottmv{n} $ &  \\
 $ \nonterm x $ & \ottcom{variable} \\
 $ \lesseqgtr $ & \ottcom{comparison} \\
}}

\newcommand{\ottfunction}{
\ottrulehead{\ottnt{function}  ,\ \nonterm f}{::=}{\ottcom{function}}\ottprodnewline
\ottfirstprodline{|}{\ottmv{fp}}{}{}{}{\ottcom{floating-point number}}\ottprodnewline
\ottprodline{|}{ x_i }{}{}{}{\ottcom{decision variable}}\ottprodnewline
\ottprodline{|}{ -  \nonterm f }{}{}{}{\ottcom{negation}}\ottprodnewline
\ottprodline{|}{\nonterm f  \ottsym{+}  \nonterm f'}{}{}{}{\ottcom{addition}}\ottprodnewline
\ottprodline{|}{\nonterm f  \ottsym{-}  \nonterm f'}{}{}{}{\ottcom{subtraction}}\ottprodnewline
\ottprodline{|}{ \nonterm f  \cdot  \nonterm f' }{}{}{}{\ottcom{multiplication}}\ottprodnewline
\ottprodline{|}{\nonterm f  \ottsym{/}  \nonterm f'}{}{}{}{\ottcom{division}}\ottprodnewline
\ottprodline{|}{ \sin  \nonterm f }{}{}{}{\ottcom{sine}}\ottprodnewline
\ottprodline{|}{ \ldots }{}{}{}{}}

\newcommand{\ottvalue}{
\ottrulehead{\ottnt{value}  ,\ \ottnt{k}  ,\ \nonterm v}{::=}{\ottcom{value}}\ottprodnewline
\ottfirstprodline{|}{\ottmv{fp}}{}{}{}{\ottcom{floating-point number}}\ottprodnewline
\ottprodline{|}{ \top }{}{}{}{\ottcom{true}}\ottprodnewline
\ottprodline{|}{ \bot }{}{}{}{\ottcom{false}}\ottprodnewline
\ottprodline{|}{\lambda  \nonterm p  \ottsym{.}  \nonterm e}{}{}{}{\ottcom{abs}}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \nonterm v_{{\mathrm{1}}}  \ottsym{,} \, ... \, \ottsym{,}  \nonterm v_{\ottmv{n}}  \ottsym{)}}{}{}{}{\ottcom{tuple}}\ottprodnewline
\ottprodline{|}{ [ \ldots [ [ v_{ij\dots 0 0}, \ldots, v_{ij\dots{}0n} ], \ldots ], \ldots ] }{}{}{}{\ottcom{array}}\ottprodnewline
\ottprodline{|}{ \left\{ k_1 \Rightarrow v_1, \dots, k_n \Rightarrow v_n \right\} }{}{}{}{\ottcom{dict}}\ottprodnewline
\ottprodline{|}{\nonterm v \, \lesseqgtr \, \nonterm v'}{}{}{}{\ottcom{comparison}}\ottprodnewline
\ottprodline{|}{\nonterm f}{}{}{}{\ottcom{function}}\ottprodnewline
\ottprodline{|}{ \sigma }{}{}{}{\ottcom{stream}}\ottprodnewline
\ottprodline{|}{\ottmv{n}}{}{}{}{\ottcom{neutral term}}\ottprodnewline
\ottprodline{|}{ \mathbf{err} }{}{}{}{\ottcom{error}}}

\newcommand{\ottexpr}{
\ottrulehead{\ottnt{expr}  ,\ \nonterm e}{::=}{\ottcom{expression}}}

\newcommand{\ottpattern}{
\ottrulehead{\ottnt{pattern}  ,\ \nonterm p}{::=}{\ottcom{pattern}}}

\newcommand{\ottgrammar}{\ottgrammartabular{
\ottfunction\ottinterrule
\ottvalue\ottinterrule
\ottexpr\ottinterrule
\ottpattern\ottafterlastrule
}}

% defnss
\newcommand{\ottdefnss}{
}

\newcommand{\ottall}{\ottmetavars\\[0pt]
\ottgrammar\\[5.0mm]
\ottdefnss}


